SoK: Differential Privacies

Shortly after it was first introduced in 2006, differential privacy became the flagship data privacy definition. Since then, numerous variants and extensions were proposed to adapt it to different scenarios and attacker models. In this work, we propose a systematic taxonomy of these variants and extensions. We list all data privacy definitions based on differential privacy, and partition them into seven categories, depending on which aspect of the original definition is modified. These categories act like dimensions: variants from the same category cannot be combined, but variants from different categories can be combined to form new definitions. We also establish a partial ordering of relative strength between these notions by summarizing existing results. Furthermore, we list which of these definitions satisfy some desirable properties, like composition, post-processing, and convexity by either providing a novel proof or collecting existing ones.

==> Appendices.tex <==
\begin{appendices}

\section{Proofs of properties}

Through the appendix, we reuse the abbreviations from Table~\ref{tab:DP_variants}.

\subsection{Axioms}

\begin{prop}[Existing Results]\label{prop:a-common}\hspace{0cm}
	\begin{enumerate}
		\item ProDP, ACoDP, and mCoDP do not satisfy the post-processing
      axiom~\cite{meiser2018approximate,bun2016concentrated}.
    \item AbsDP satisfies neither privacy axiom, while GlDP satisfies
      both~\cite{kifer2010towards,kifer2012rigorous}\footnote{As an immediate
      corollary, all definitions which combine notions in \textbf{N} and NPr
      also satisfy both axioms.}.
    \item WBDP satisfies the post-processing axiom~\cite{triastcyn2019bayesian}.
    \item TypSt satisfies the post-processing axiom~\cite{bassily2016typical}.
    \item Gauss DP satisfies the post-processing axiom~\cite{dong2019gaussian}.
		\item PFPr satisfy both privacy axioms~\cite{kifer2012rigorous}.
		\item CWPr satisfy both privacy axioms~\footnote{As an immediate corollary,
      DistDP and ZKPr also satisfy both axioms.}~\cite{bassily2013coupled}.
    \item APKDP and PPKDP satisfy both privacy
      axioms~\cite{desfontaines2019differential}.
    \item BLDP satisfies both privacy axioms~\cite{ligett2020bounded}.
	\end{enumerate}
\end{prop}

\begin{prop}\label{prop:a-div}
  All instantiations of DivDP satisfy both privacy axioms. In particular,
  approximate DP, MIDP, KLPr, RenDP, and zCoDP satisfy both axioms.
  \begin{proof}
    The post-processing axiom follows directly from the monotonicity property of
    the $f$-divergence. The convexity axiom follows directly from the joint
    convexity property of the $f$-divergence.
  \end{proof}
\end{prop}

\begin{prop}\label{prop:a-c-prob}
  ProDP and ACoDP do not satisfy the convexity axiom.
  \begin{proof}
    Consider the following mechanisms $\mecha_1$ and $\mecha_2$, with input and
    output in $\{0,1\}$.
    \begin{itemize}
    \item $\mechone{0}=0$, $\mechone{1}=1$ with probability $\del$, and
      $\mechone{1}=0$ with probability $1-\del$.
    \item $\mechtwo{0}=\mechtwo{1}=1$.
    \end{itemize}
    Both mechanisms are $\left(\frac{1}{1-\del},\del\right)$-ProDP\@. Now,
    consider the mechanism $\mecha$ which applies $\mecha_1$ with probability
    $1-2\del$ and $\mecha_2$ with probability $2\del$. $\mecha$ is a convex
    combination of $\mecha_1$ and $\mecha_2$, but the reader can verify that it
    is not $\left(\frac{1}{1-\del},\del\right)$-ProDP\@. The result for
    $(\xi,\rho,\del)$-ACoDP is a direct corollary, since is is equivalent to
    $(\xi,\del)$-ProDP when $\rho=0$.
  \end{proof}
\end{prop}

\begin{prop}\label{prop:a-d}
  $d_\datasets$-Pr satisfies both privacy axioms. Further, EDivDP also satisfies
  both privacy axioms.
  \begin{proof}
    The proof of Proposition~\ref{prop:a-common} for PFPr (Appendix~B
    in~\cite{kifer2012rigorous}) is a proof by case analysis on every possible
    protected property. The fact that $\eps$ is the same for every protected
    property has no influence on the proof, so we can directly adapt the proof
    to $d_\datasets$-Pr, and its combination with PFPr.
    Similarly, the proof can be extended to arbitrary divergence functions, like
    in Proposition~\ref{prop:a-div}.
  \end{proof}
\end{prop}

\begin{prop}\label{prop:a-c-rand}
  RanDP does not satisfy the convexity axiom.
  \begin{proof}
    Let $\pi$ be the uniform distribution on $\{0,1\}$, let $D_1$ be generated
    by picking $10$ records according to $\pi$, and $D_2$ by flipping one record
    at random. Let $\mecha_0$ return $0$ if all records are $0$, and $\bot$
    otherwise. Let $\mecha_1$ return $1$ if all records are $1$, and $\bot$
    otherwise.
    
    Note that both mechanisms are $(\pi,2^{-9},0)$-RanDP\@. Indeed, $\mecha_0$
    will only return $0$ for $D_1$ with probability $2^{-10}$, and for $D_2$
    with probability $2^{-10}$ (if $D_1$ only has one $1$, which happens with
    probability $10\cdot2^{-10}$, and this record is flipped, which happens with
    probability $0.1$). In both cases, $\mecha_0$ will return $\bot$ for the
    other database; which will be a distinguishing event. Otherwise, $\mecha_0$
    will return $\tau$ for both databases, so $\mech{D_1}\ind_0\mech{D_2}$. The
    reasoning is the same for $\mecha_1$. 
    
    However, the mechanism $\mecha_{0.5}$ obtained by applying either $\mecha_0$
    or $\mecha_1$ uniformly randomly doesn't satisfy $(\pi,2^{-9},0)$-RanDP\@:
    the indinguishability property does not hold if $D_1$ or $D_2$ have all
    their records set to \emph{either} $0$ or $1$, which happens twice as often
    as either option alone.
  \end{proof}
\end{prop}

\begin{prop}\label{prop:a-def}
  All variants of MPr, AdvPr, and ANPr satisfy both axioms. As a direct
  corollary, InfPr also satisfies both axioms.
  \begin{proof}
    We prove it for AdvPr. A mechanism $\mecha$ satisfies $\Thepsdel$-AdvPr if
    for all $t\in\tuples$, $\theta\in\Theta$, and $S\subseteq\outputs$,
    $\probasc{D\sim\theta}{t\in D}{\mech{D}\in S}\le e^\eps\cdot\probas{D\sim\theta}{t\in D}+\del$.
    We first prove that it satisfies the convexity axiom. Suppose $\mecha$ is a
    convex combination of $\mecha_1$ and $\mecha_2$. Simplifying
    $\probas{D\sim\theta}{\dots}$ into $\proba{\dots}$, we have:
    \begin{align*}
      & \probac{t\in D}{\mech{D}\in S} = \\
      & \qquad\frac{\proba{t\in D\text{ and }\mech{D}\in S\text{ and }\mecha=\mecha_1}}{\proba{\mech{D}\in S}}
      + \frac{\proba{t\in D\text{ and }\mech{D}\in S\text{ and }\mecha=\mecha_2}}{\proba{\mech{D}\in S}} \\
    \end{align*}
    Denoting $X_i=\proba{\mech{D}\in S\text{ and }\mecha=\mecha_i}$ for $i\in\{1,2\}$, this gives:
    \begin{align*}
      \probac{t\in D}{\mech{D}\in S}=
      \frac{X_1\cdot\probac{t\in D}{\mechone{D}\in S}}{X_1+X_2}
      \frac{X_2\cdot\probac{t\in D}{\mechtwo{D}\in S}}{X_1+X_2} \\
      \le \frac{X_1\left(e^\eps\cdot\proba{t\in D}\right)+\del}{X_1+X_2}
      + \frac{X_2\left(e^\eps\cdot\proba{t\in D}\right)+\del}{X_1+X_2}
      \le e^\eps\cdot\proba{t\in D} + \del.
    \end{align*}
    The proof for the post-processing axiom is similar, summing over all
    possible outputs $\mech{D}$. It is straightforward to adapt the proof to
    all other definitions which change the shape of the prior-posterior bounds.
  \end{proof}
\end{prop}

\begin{prop}\label{prop:a-comp}
  Both versions of CDP satisfy both privacy axioms; where the post-processing
  axiom is modified to only allow post-processing with functions computable on a
  probabilistic polynomial time Turing machine. As a direct corollary of
  Proposition~\ref{prop:a-common} for CWPr, CZKPr also satisfies both privacy axioms.
  \begin{proof}
    For Ind-CDP and the post-processing axiom, the proof is straightforward: if
    post-processing the output could break the $\eps$-indistinguishability
    property, the attacker could do this on the original output and break the
    $\eps$-indistinguishability property of the original definition.
    
    For Ind-CDP and the convexity axiom, without loss of generality, we can
    assume that the sets of possible outputs of both mechanisms are disjoint
    (otherwise, this give strictly less information to the attacker). The proof
    is then the same as for the post-processing axiom.
    
    For SimCDP, applying the same post-processing function to the ``true''
    differentially private mechanism immediately leads to the result, since DP
    satisfies post-processing. The same reasoning holds for convexity.
  \end{proof}
\end{prop}

\subsection{Composition}

In this section, if $\mecha_1$ and $\mecha_2$ are two mechanisms, we denote
$\mecha_{1+2}$ the mechanism defined by
$\mecha_{1+2}(D)=\left(\mecha_1(D),\mecha_2(D)\right)$.

\begin{prop}[Existing Results]\label{prop:c-common}
If $\mecha_1$ and $\mecha_2$ are respectively\ldots
  \begin{enumerate}
    \item $\left(\eps_1,\del_1\right)$-DP and $\left(\eps_2,\del_2\right)$-DP,
      then $\mecha_{1+2}$ is $\left(\eps_1+\eps_2,\del_1+\del_2\right)$-DP~\cite{dwork2006our}.
    \item $\left(\eps_1,\del_1\right)$-ProDP and $\left(\eps_2,\del_2\right)$-ProDP,
      then $\mecha_{1+2}$ is $\left(\eps_1+\eps_2,\del_1+\del_2\right)$-ProDP~\cite{machanavajjhala2008privacy,canard2015differential,meiser2018approximate}.
    \item $\left(\eps_1,\del_{a,1},\del_{p,1}\right)$-RelDP and
      $\left(\eps_2,\del_{a,2},\del_{p,2}\right)$-RelDP,
      then $\mecha_{1+2}$ is
      $\left(\eps_1+\eps_2,\del_{a,1}+\del_{a,2},\del_{p,1}+\del_{p,2}\right)$-RelDP~\cite{zhang2015toward}.
    \item $\eps_1$-MIDP and $\eps_2$-MIDP, then $\mecha_{1+2}$ is
      $\left(\eps_1+\eps_2\right)$-MIDP~\cite{cuff2016differential}.
    \item $\eps_1$-KLDP and $\eps_2$-KLDP, then $\mecha_{1+2}$ is
      $\left(\eps_1+\eps_2\right)$-KLDP~\cite{barber2014privacy,cuff2016differential}.
    \item $\left(\alpha_1,\eps_1\right)$-RenDP and $\left(\alpha_2,\eps_2\right)$-RenDP,
      then $\mecha_{1+2}$ is
      $\left(\max\left(\alpha_1,\alpha_2\right),\eps_1+\eps_2\right)$-RenDP~\cite{mironov2017renyi}.
    \item $\left(\mu_1,\tau_1\right)$-mCoDP and
      $\left(\mu_2,\tau_2\right)$-mCoDP, then $\mecha_{1+2}$ is
      $\left(\mu_1+\mu_2,\sqrt{{\mu_1}^2+{\mu_2}^2}\right)$-mCoDP~\cite{dwork2016concentrated,bun2016concentrated}.
    \item $\left(\xi_1,\rho_1\right)$-zCoDP and
      $\left(\xi_2,\rho_2\right)$-zCoDP, then $\mecha_{1+2}$ is
      $\left(\xi_1+\xi_2,\xi_1+\xi_2\right)$-zCoDP~\cite{bun2016concentrated}.
    \item $\left(\xi_1,\rho_1,\del_1\right)$-ACoDP and
      $\left(\xi_2,\rho_2,\del_2\right)$-ACoDP, then $\mecha_{1+2}$ is
      $\left(\xi_1+\xi_2,\xi_1+\xi_2,\del_1+\del_2-\del_1\del_2\right)$-ACoDP~\cite{bun2016concentrated}.
    \item $\left(\xi_1,\rho_1,\omega_1\right)$-bCoDP and
      $\left(\xi_2,\rho_2,\omega_2\right)$-bCoDP, then $\mecha_{1+2}$ is
      $\left(\xi_1+\xi_2,\xi_1+\xi_2,\min(\omega_1,\omega_2)\right)$-bCoDP~\cite{bun2016concentrated}.
    \item $\left(\eta_1,\tau_1\right)$-CCoDP and
      $\left(\eta_2,\tau_2\right)$-CCoDP, then $\mecha_{1+2}$ is
      $\left(\eta_1+\eta_2,\frac{{\eta_1+\eta_2}^2}{2}\right)$-CCoDP~\cite{colisson2016l3}.
    \item $f_1$-DP and $f_2$-DP, than then $\mecha_{1+2}$ is $f_1\otimes
      f_2$-DP~\cite{dong2019gaussian}.
    \item $(\pi,\gamma_1,\eps_1)$-RanDP and $(\pi,\gamma_2,\eps_2)$-RanDP, then 
      $\mecha_{1+2}$ is
      $(\pi,\gamma_1+\gamma_2,\eps_1+\eps_2)$-RanDP~\cite{hall2012new}.
    \item $\left(\pi,\eps_1,\del_1\right)$-BayDP\textsuperscript{\cite{triastcyn2019bayesian}}
      and $\left(\pi,\eps_1,\del_1\right)$-BayDP\textsuperscript{\cite{triastcyn2019bayesian}},
      then $\mecha_{1+2}$ is
      $\left(\pi,\eps_1+\eps_2,\del_1+\del_2\right)$-BayDP\textsuperscript{\cite{triastcyn2019bayesian}}.
      The same result holds for WBDP as an immediate consequence of Theorem~1
      in~\cite{triastcyn2019bayesian}.
    \item $(\Theta,\eps_1,\gamma_1,\del_1)$-TypSt and
      $(\Theta,\eps_2,\gamma_2,\del_2)$-TypSt, then $\mecha_{1+2}$ is
      $(\Theta,\eps_1+\eps_2,\gamma_1+\gamma_2,\del_1+\del_2)$-TypSt~\cite{bassily2016typical}.
    \item $(d_\datasets,\eps_1,\del_1)$-PsDP and
      $(d_\datasets,\eps_2,\del_2)$-PsDP then $\mecha_{1+2}$ is
      $(d_\datasets,\eps_1+\eps_2,\del_1+\del_2)$-PsM
      DP~\cite{dimitrakakis2013bayesian}.
    \item $(P_1,\eps_1,\del_1)$-BLDP and $(P_2,\eps_2,\del_2)$-BLDP, then
      $\mecha{1+2}$ is $(P_{1+2},\eps_1+\eps_2,\del_1+\del_2)$-BLDP, where
      $P_{1+2}$ is the concatenation of $P_1$ and $P_2$ (where the randomness
      is not shared between $P_1$ and $P_2$, nor between $\mecha_1$ and
      $\mecha_2$)~\cite{ligett2020bounded}.
  \end{enumerate}
\end{prop}

\begin{prop}\label{prop:c-d}
  If $\mecha_1$ is $d^1_\datasets$-private and $\mecha_2$ is
  $d^2_\datasets$-private, then $\mecha_{1+2}$ is $d^{1+2}_\datasets$-private,
  where
  $d^{1+2}_\datasets\left(D_1,D_2\right)=d^1_\datasets\left(D_1,D_2\right)+d^2_\datasets\left(D_1,D_2\right)$.
  \begin{proof}
    The proof is essentially the same as for $\eps$-DP\@. $\mecha_1$'s
    randomness is independent from $\mecha_2$'s, so:
    
    \begin{equation*}
    \begin{gathered}
      \proba{\mechone{D_1}=O_1~\text{and}~\mechtwo{D_1}=O_2}=
      \proba{\mechone{D_1}=O_1}\cdot\proba{\mechtwo{D_1}=O_2}\\
      \le e^{d^1_\datasets\left(D_1,D_2\right)}\cdot\proba{\mechtwo{D_2}=O_1}
      \cdot e^{d^2_\datasets\left(D_1,D_2\right)}\cdot\proba{\mechtwo{D_2}=O_2} \\
      \le e^{d^{1+2}_\datasets\left(D_1,D_2\right)}
                    \cdot\proba{\mechone{D_2}=O_1~\text{and}~\mechtwo{D_2}=O_2}.
    \end{gathered}
    \end{equation*}
    
    Each definition listed in Proposition~\ref{prop:c-common} can also be
    combined with $d_\datasets$-privacy, and the composition proofs can be
    similarly adapted.
  \end{proof}
\end{prop}

\begin{prop}\label{prop:c-b}
  In general, definitions which assume limited background knowledge from the
  adversary do not compose.
  \begin{proof}
    The proof of Proposition~\ref{prop:c-d} cannot be adapted to a context in
    which the attacker has limited background knowledge: as the randomness
    partially comes from the data-generating distribution, the two probabilities
    are no longer independent. A typical example considers two mechanisms which
    answer e.g., queries ``how many records satisfy property $P$'' and ``how many
    records satisfy property $P$ and have an ID different from 4217'': the
    randomness in the data might make each query private, but the combination of
    two queries trivially reveals something about a particular user. Variants of
    this proof can easily be obtained for all definitions with limited
    background knowledge.
  \end{proof}
\end{prop}

%\section{Relations between definitions in \textbf{Q}}\label{sec:q-rel}

%\begin{table}[!h]
%    \centering
%    \begin{tabular}{l}
%        \toprule
%        {}\cite{colisson2016l3,bun2016concentrated,bun2018composable}: \\
%        $(\eta,\tau)$-CCoDP $\Leftrightarrow$ $\eta$-DP \\
%        $\eps$-DP $\Leftrightarrow$ $(\eps,\eps^2/2)$-CCoDP \\
%        $(\eta,\tau)$-CCoDP $\Rightarrow$ $(0,\tau)$-zCoDP \\
%        $(\xi,\rho)$-zCoDP $\Rightarrow$ $(\infty,\rho)$-CCoDP \\
%        $\rho$-zCoDP $\Leftrightarrow$ $(\rho,\infty)$-tCoDP \\
%        $(\xi,\rho)$-zCoDP $\Leftrightarrow$ $(\xi,\rho,\infty)$-bCoDP \\
%        $(\eta,\tau)$-CCoDP $\Rightarrow$ $(\min(\eta,\tau),\eta+\min(\eta,\tau)/2)$-mCoDP \\
%        \midrule
%        %$(0,\del)$-DP $\Rightarrow$ $2h(\del)+2\del\log[\min\{|\outputs|,\max\{|\datasets|+1\}\}]$-MI-DP\footnote{$h(\cdot)$ is the binary entropy function.} (Lemma 3 in~\cite{cuff2016differential}) \\
%        \midrule

%        %$(\xi,\rho)$-zCoDP $\Longleftrightarrow$ $\forall\alpha:(\xi+\rho\alpha)$-R\'enDP (Implied by the definitions) \\

%        %$\epsdel$-DP $\Rightarrow$ $\del$ approximate $\frac{\eps^2}{2}$-zCoDP (Corollary 8.7 in~\cite{bun2016concentrated}) \\
%        %$\del$ approximate $(\eps,0)$-zCoDP $\Rightarrow$ $\epsdel$-DP (Corollary 8.7 in~\cite{bun2016concentrated}) \\
%    \end{tabular}
%    \caption{Relations between definitions in \textbf{Q}}\label{tab:q-rel}
%\end{table}

\end{appendices}

